Evaluating the effect of stellar multiplicity on the PSF of space-based weak lensing surveys

The next generation of space-based telescopes used for weak lensing surveys will require exquisite point spread function (PSF) determination. Previously negligible effects may become important in the reconstruction of the PSF, in part because of the improved spatial resolution. In this paper, we show that unresolved multiple star systems can affect the ellipticity and size of the PSF and that this effect is not cancelled even when using many stars in the reconstruction process. We estimate the error in the reconstruction of the PSF due to the binaries in the star sample both analytically and with image simulations for different PSFs and stellar populations. The simulations support our analytical finding that the error on the size of the PSF is a function of the multiple stars distribution and of the intrinsic value of the size of the PSF, i.e. if all stars were single. Similarly, the modification of each of the complex ellipticity components (e1,e2) depends on the distribution of multiple stars and on the intrinsic complex ellipticity. Using image simulations, we also show that the predicted error in the PSF shape is a theoretical limit that can be reached only if large number of stars (up to thousands) are used together to build the PSF at any desired spatial position. For a lower number of stars, the PSF reconstruction is worse. Finally, we compute the effect of binarity for different stellar magnitudes and show that bright stars alter the PSF size and ellipticity more than faint stars. This may affect the design of PSF calibration strategies and the choice of the related calibration fields.

==> description_binary_formation.tex <==
\subsection{Formation of Multiple Systems}
Star formation occur by fragmentation and collapse to the local Jeans mass of molecular clouds. Molecular clouds fragment to create region of higher density which lead to the formation of proto-stars by accretion of gas and dust to central regions of the fragments.
Numerical simple hydrodynamical studies \citep{Bate2009} of the collapse of unstable -- large ratio of mass to Jeans mass -- and turbulent clouds lead to the right proportion of multiple systems. This would indicate that formation of multiple system is a common enough event \citep{Reipurth2014}.

Close binaries -- i.e. with semimajor axis $\sim 100$ AU -- tend to form from orbital decay of wider binaries through dynamical interaction, accretion and interaction of with the proto-stellar disks \citep{Bate2012}. The orbital decay of the wide binaries to closer-in systems theoretically suggests that very wide binaries (separations $\sim 1000$ AU and larger) represent a small portion of the multiple system population.

Due to gravitational interactions, ejections or capture of system members is a possibility. Multiple systems that contain members that differ greatly in mass are less dynamically stable than same mass members systems and will eject some of the companion during the secular evolution of the system. Close multiple system exhibit thus very similar masses, because too light members would have been ejected from the system by the time they become T Tauri stars \citep{White2001}.
Hierarchical system can be created by those interactions and by collapse of nearby fragments of the molecular cloud. All hierarchical system members do not orbit about the same centre of mass. An example would be a system of binaries that is made of two objects with large separation. One of the object is a star whilst the other is a close binary system.
